Attentive Social Recommendation: Towards User And Item Diversities

Social recommendation system is to predict unobserved user-item rating values by taking advantage of user-user social relation and user-item ratings. However, user/item diversities in social recommendations are not well utilized in the literature. Especially, inter-factor (social and rating factors) relations and distinct rating values need taking into more consideration. In this paper, we propose an attentive social recommendation system (ASR) to address this issue from two aspects. First, in ASR, Rec-conv graph network layers are proposed to extract the social factor, user-rating and item-rated factors and then automatically assign contribution weights to aggregate these factors into the user/item embedding vectors. Second, a disentangling strategy is applied for diverse rating values. Extensive experiments on benchmarks demonstrate the effectiveness and advantages of our ASR.

==> Algorithm.tex <==
\section{Objective Function} %and Algorithm
\label{sec:alg}
To predict the the value of unobserved rating user $x$ on item $y$, we first concatenate the latent user/item factors from the last Rec-conv layer, i.e. $\mathbf{u}_x^{(L)}$ and $\mathbf{i}_y^{(L)}$. We then feed the concatenation $[\mathbf{u}_x^{(L)} \oplus \mathbf{i}_y^{(L)}]$ into MLP to predict the rating value. Mean square error is adopted as the objective function:
\begin{equation}
    \label{eq:objective}
    Loss = \frac{1}{2|\mathcal{R}|}\sum_{(x,y)\in \mathcal{R}}(r'_{xy}-r_{xy})^2
\end{equation}
Here, $\mathcal{R}$ is the set of observed user-item ratings, and $r'_{xy}$ is the predicted value.


==> others.tex <==
\section{others}
\begin{figure}[!t]
    \centering
    \subfigure[Ciao]{\includegraphics[width=1.6in]{Figure/Exp/ciao_distribution.eps}\label{fig:gt:dis}}
    \subfigure[Ranking]{\includegraphics[width=1.6in]{Figure/Exp/ciao_distribution2.eps}\label{fig:density}}
        \subfigure[Ciao]{\includegraphics[width=1.6in]{Figure/Exp/ciao_distribution_l2.eps}\label{fig:density}}
    \caption{Score Distributions of Ciao}
    \label{fig:para:l}
\end{figure}

==> review.tex <==
\section*{Reviews}

\subsection{Review 1}
The authors propose an attentive social recommendation model for item recommendation with social networks. In particular, their model consists of three factors, namely the user factor, the social factor, and the user-item factor, where the latter two factors are computed from the social network and the user-item rating bipartite graph respectively. To incorporate multiple factors in a united model, the authors adopt the attention mechanism to learn a weighting scheme for each user. Although simple, there exist several issues in this work, as follows.

\textcolor{red}{(1) This work is kind of incremental to previous work, such as DANSER (WWW’19) and GraphRec (WWW’19), which already integrate multiple data sources in their models.}

\textcolor{green}{(2) Some relevant works are missing in the discussion of related work for social recommendation, e.g., the followings, which render it difficult to be convinced with the novelty of the proposed method.
Le Wu, Peijie Sun, Yanjie Fu, Richang Hong, Xiting Wang, Meng Wang: A Neural Influence Diffusion Model for Social Recommendation. SIGIR 2019: 235-244
Weiping Song, Zhiping Xiao, Yifan Wang, Laurent Charlin, Ming Zhang, Jian Tang: Session-Based Social Recommendation via Dynamic Graph Attention Networks. WSDM 2019: 555-563}

\textcolor{blue}{(3) There are many sub-modules in the model, each of which contains expensive calculations and produces giant results, resulting in high costs in both time and space. The authors should demonstrate the performance of the proposed method in some large datasets, which are the cases in real-life applications, instead of only two small datasets.}

\textcolor{red}{(4) Several formulas are provided directly without proper explanations on the intuition or principles behind them.}

\textcolor{blue}{(5) The quality of presentation is far from the expectation with several typos (e.g., “An user-item pair” and “Socia”) and duplicate paragraphs (e.g., the introduction of baselines in Section 5.1 are similar to the one in related work section).}


\subsection{Review 2}
Questions
1. Overall score
Weak Reject (marginally below the acceptance threshold. Accepting it would not be that bad)
4. Comments to authors

Authors propose an attentive graph neural network, which makes a social recommendation from item-centric and user-centric effects. And they conduct various experiments.

\textcolor{red}{1. The definitions of 'intra-factor' and 'inter-factor' are not clear. The examples of 'song' and 'computer' make me difficult to understand intra-factor and inter-factor.}

\textcolor{green}{2. There may be some mistakes in Figure.2(b). As shown in Eq.(7), $I^(l,u->i,k)$ is calculated by $R_k$ and $U^(l)$. But there are no arrows from $U^(l)$ to $I^(l,u->i,k)$. The same mistake arose in Eq.(3).}

\textcolor{blue}{3. Authors use P-ACC as a ranking metric. Why not using NDCG, which is a widely used metric to evaluate the ranking performance on each user?}

\textcolor{red}{4. Why did SVD++ perform worse than UserMean and ItemMean? The authors should explain the results in more detail. --- Refer to the SIGIR paper for description}

\textcolor{red}{5. The authors analyze the impacts of disentangling strategy. It will be better to use some visualizations i.e., the effect of rating levels for a user.}

Authors need to improve written for two reasons.

\textcolor{red}{1) It costs me a lot of time to understand the relationship between the fourth paragraph and the sixth paragraph, which introduces the shortcomings of related work and challenges in this paper.
2) The paragraphs which introduce the proposed model(para.6,7,8) need to be reorganized.}

\subsection{Review 3}
There are a few incorrect claims in the related work and introduction. "First, existing works overlook distinct interfactor contributions." - two important threads of work in social recommendation are missed here, social exposure modeling for recommendation:

Wang, Menghan, et al. "Collaborative filtering with social exposure: A modular approach to social recommendation." Thirty-Second AAAI Conference on Artificial Intelligence. 2018.

Chen, Jiawei, et al. "Modeling Users' Exposure with Social Knowledge Influence and Consumption Influence for Recommendation." Proceedings of the 27th ACM International Conference on Information and Knowledge Management. 2018.

\textcolor{blue}{and adversarial modeling for social recommendation:}

Krishnan, Adit, et al. "A modular adversarial approach to social recommendation." Proceedings of the 28th ACM International Conference on Information and Knowledge Management. 2019.

Fan, Wenqi, et al. "Deep adversarial social recommendation." arXiv preprint arXiv:1905.13160 (2019).

\textcolor{blue}{Both the above frameworks are capable of including cross-factor associations and contextual weighting. It is important to compare these threads on a conceptual level and in terms of performance, if possible.}

The proposed method incorporates user side, item side and user-item propagation, and thus involves a large number of graph convolution steps, with projected graphs for each rating value. 
This strategy has two weaknesses - first, it scales poorly owing to the large number of graph networks and parameters of the channels, and further, 

\textcolor{red}{it makes the assumption that each rating value has consistent semantics across users and items. Past work has shown that relative ratings (e.g., how does a rating differ from the user's or item's average, instead of the absolute value) are quite important. Thus inducing graphs on absolute rating values may result in inconsistent semantics since some users may rate many items high, while others may be more selective. Such bias should be accounted.---- Eq. (3), for the same rating-$k$ $W^{(k)}$ is shared among different users}

The most important steps to improve the presented work are to conceptually distinguish the proposed framework against the additional threads of related work pointed above. It also appears that the rating semantics and model scalability might be addressed together - do we really need K different GCNs? The authors could consider developing a GCN like edge propagation model based on the relative importance of each edge of a user or item, accounting for diverse rating value semantics as well as avoiding the O(K) scaling. \textcolor{blue}{Add GAT description in the end of Sec 4.1.2 (GAT is also applied which considers different rating values with different effects but we found that disentangling GCN has better performance. Please refer to Sec 5.4.3 )}


\subsection{Review 4}
This paper proposes an attentive social recommendation system ASR, which captures the intra- and inter-factor features from both social and rating graphs. Experiments on real-world datasets demonstrate the effectiveness of ASR over state-of-the arts. However, I have the following concerns:

\textcolor{blue}{1. The example in the Introduction is not consistent with the datasets used in the paper. As shown in Figure 1, the authors structure the user social graph as an undirected graph, while the Ciao and Epinion datasets consist of directed social relations. There is no illustration about the construction of social graph for two datasets, and thus my major concern is if the directed social relations are treated as undirected relations in the experiments.--- modify in Sec 5.1.1}

\textcolor{blue}{2. The intra-factor of social factor has not been well explored. In section 4.1.1, the user social vector is generated by applying a GCN on the social graph, which only considers the local neighbors and meanwhile ignores the influence of social relation strength. Therefore, I suppose this paper fails to sufficiently explore the social information for predicting user preference.---- Footnote 1 is not clear. Add a ablation study}

\textcolor{blue}{3. The inter-factor contributions between user-rating and item-rated factor have not been explicitly investigated. As claimed in the introduction, the two factors should have varying contributions on user preference when recommending items with different categories. However, the proposed attention aggregation only balances the user-social and user-rating factors, while cannot explicitly distinguish the dynamic contribution of user-rating and item-rated factors.----add case study visualization}

\textcolor{red}{4. This paper exploits the rating scores to improve recommendation performance, while we may only have implicit feedback available in practice.}

\textcolor{blue}{5. There is no complexity analysis of the proposed model, and it would be better to show the detailed results of significance tests. Besides, as shown in Figure 4, the item attention mechanism contributes more to performance than user attention, and the reasons for this observation should be further explained.----add a table of parameter size}



\section{To do list}
\begin{itemize}
    % \item reference
    % \item figure 2.b more clear
    \item add a table of parameter size or running time per epoch
    \item add a ablation study: replace GCN with GAT in social graph (Review 4 (2))
    \item P-ACC results
\end{itemize}

==> symbol.tex <==
\begin{Huge}
\newpage
$$
\mathbf{A}^{(l,u)}
$$

$$
\mathbf{A}^{(l,\mathcal{U}\rightarrow u)}
$$

$$
\mathbf{A}^{(l,\mathcal{I}\rightarrow u)}
$$

$$
\mathbf{B}^{(l,i)}
$$


$$
\mathbf{B}^{(l,\mathcal{U}\rightarrow i)}
$$

$$
\mathbf{U}^{(0)}
$$

$$
\mathbf{U}^{(1)}
$$

$$
\mathbf{U}^{(l,\mathcal{U}\rightarrow u)}
$$

$$
\mathbf{U}^{(l,\mathcal{I}\rightarrow u)}
$$


% $$
% \mathbf{I}^{(0)}
% $$

$$
\mathbf{I}^{(l,\mathcal{U}\rightarrow i)}
$$

% $$
% \mathbf{I}^{(1)}
% $$

% $$
% \mathbf{U}^{(0)}
% $$

% $$
% \mathbf{U}^{(0,i\rightarrow u)}
% $$

% $$
% \mathbf{U}^{(0,u\rightarrow u)}
% $$

% $$
% \mathbf{A}^{(0,u)}
% $$

% $$
% \mathbf{W}^{(0,u)}_{A}
% $$

\end{Huge}


% \begin{align*}
% \mathbf{U}^{(l+1)}  &= \mathbf{U}^{(l)}\odot(\mathbf{A}^{(l,u)})+\mathbf{U}^{(l,u\rightarrow u)}\odot\mathbf{A}^{(l,u\rightarrow u)}\\
%                         &+\mathbf{U}^{(l,i\rightarrow u)}\odot\mathbf{A}^{(l,i\rightarrow u)}
% \end{align*}

% \ouru: $\mathbf{A}^{(l,u)}=0, \mathbf{A}^{(l,i\rightarrow u)}=1, \mathbf{U}^{(l,i\rightarrow u)}=1$
